Solving Inverse Problems with Latent Diffusion Models via Hard Data Consistency

Diffusion models have recently emerged as powerful generative priors for solving inverse problems. However, training diffusion models in the pixel space are both data-intensive and computationally demanding, which restricts their applicability as priors for high-dimensional real-world data such as medical images. Latent diffusion models, which operate in a much lower-dimensional space, offer a solution to these challenges. However, incorporating latent diffusion models to solve inverse problems remains a challenging problem due to the nonlinearity of the encoder and decoder. To address these issues, we propose \textit{ReSample}, an algorithm that can solve general inverse problems with pre-trained latent diffusion models. Our algorithm incorporates data consistency by solving an optimization problem during the reverse sampling process, a concept that we term as hard data consistency. Upon solving this optimization problem, we propose a novel resampling scheme to map the measurement-consistent sample back onto the noisy data manifold and theoretically demonstrate its benefits. Lastly, we apply our algorithm to solve a wide range of linear and nonlinear inverse problems in both natural and medical images, demonstrating that our approach outperforms existing state-of-the-art approaches, including those based on pixel-space diffusion models.

==> ReSample_arixv417/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ReSample_arixv417/text/algorithm.tex <==
\section{ReSample: Inverse Problems using Latent Diffusion Models}
\label{sec:resample}


%In this section, we discuss our proposed algorithm ReSample and how it can resolve the issues raised by Latent-DPS. In Section~\ref{sec:prop}, we discuss our algorithm in more detail and in Section~\ref{sec:theory}, we develop a theory to rigorously argue the benefits of our approach.


%%%% =========
\subsection{Proposed Method}
\label{sec:prop}

\paragraph{Hard Data Consistency.} Similar to Latent-DPS, our algorithm involves incorporating data consistency into the reverse sampling process of LDMs. However, instead of a gradient-like update as shown in Equation~(\ref{eq:latent_dps_gradient}), we propose to solve an optimization problem on \emph{some time steps $t$} of the reverse process:
\begin{align}
\label{eq:hard_data_consistency}
    \hat{\bm{z}}_0(\bm{y}) \in \underset{\bm{z}}{\argmin} \, \frac{1}{2} \| \bm{y} - \mathcal{A}(\mathcal{D}(\bm{z})) \|^2_2,
\end{align}
where we denote $\hat{\bm{z}}_0(\bm{y})$ as the sample consistent with the measurements $\bm{y} \in \R^m$. This optimization problem has been previously explored in other works that use GANs for solving inverse problems, and can be efficiently solved using iterative solvers such as gradient descent~\cite{csgm, robust_csgm, shah2021provably, dip}. However, it is well known that solving this problem starting from a random initial point may lead to unfavorable local minima~\cite{csgm}. To address this, we solve Equation~(\ref{eq:hard_data_consistency}) starting from an initial point $\hat{\bm{z}}_0(\bm{z}_{t+1})$, where $\hat{\bm{z}}_0(\bm{z}_{t+1})$ is the estimate of ground-truth latent vector at time $0$ based on the sample at time $t+1$. 
%One can solve Equation~(\ref{eq:hard_data_consistency}) using iterative solvers such as gradient descent, but instead of starting at some random initial point, we initialize using $\hat{\bm{z}}_0(\bm{z}_t)$, where $\hat{\bm{z}}_0(\bm{z}_t)$ is an estimate of the ground-truth latent sample at time $t$. 
The intuition behind this initialization is that we want to start the optimization process within local proximity of the global solution of Equation~(\ref{eq:hard_data_consistency}), to prevent resulting in a local minimum. We term this overall concept as \emph{hard data consistency}, as we strictly enforce the measurements via optimization, rather than a ``soft'' approach through gradient update like Latent-DPS.
To obtain $\hat{\bm{z}}_0(\bm{z}_{t+1})$, we use Tweedie's formula~\cite{tweedie} that gives us an approximation of the posterior mean which takes the following formula:
\begin{align}
    \hat{\bm{z}}_0(\bm{z}_t) = \mbb{E}[\bm{z}_0 | \bm{z}_{t}] = \frac{1}{\sqrt{\bar{\alpha}_{t}}} (\bm{z}_{t} + (1-\bar{\alpha}_{t})\nabla \log p(\bm{z}_{t})).
\end{align}

However, we would like to note that performing hard data consistency on every reverse sampling iteration $t$ may be very costly. To address this, we first observe that as we approach $t=T$, the estimated $\hat{\bm{z}}_0(\bm{z}_t)$ can deviate significantly from the ground truth. In this regime, we find that hard data consistency provides only marginal benefits. Additionally, in the literature, existing works 
% that incorporate conditional diffusion models 
point out the existence of a three-stage phenomenon~\cite{freedom}, where they demonstrate that data consistency is primarily beneficial for the semantic and refinement stages (the latter two stages when $t$ is closer to $0$) of the sampling process.
Following this reasoning, we divide $T$ into three sub-intervals and only apply the optimization in the latter two intervals. This approach provides both computational efficiency and accurate estimates of $\hat{\bm{z}}_0(\bm{z}_t)$.



Furthermore, even during these two intervals, we observe that we do not need to solve the optimization problem on every iteration $t$. Because of the continuity of the sampling process, after each data-consistency optimization step, the samples in the following steps can still remain similar semantic or structural information to some extent. Thus, we ``reinforce'' the data consistency constraint during the sampling process via a skipped-step mechanism. Empirically, we see that it is sufficient to perform this on every $10$ (or so) iterations of $t$. One can think of hard data consistency as guiding the sampling process towards the ground truth signal $\bm{x}^*$ (or respectively $\bm{z}^*$) such that it is consistent with the given measurements.
Lastly, in the presence of measurement noise, minimizing Equation~(\ref{eq:hard_data_consistency}) to zero loss can lead to overfitting the noise. To remedy this, we perform early stopping, where we only minimize up to a threshold $\tau$ based on the noise level. We will discuss the details of the optimization process in the Appendix. We also observe that an additional Latent-DPS step after unconditional sampling can (sometimes) marginally increase the overall performance. We perform an ablation study on the performance of including Latent-DPS in the Appendix.



\begin{algorithm}[t]
\caption{ReSample: Solving Inverse Problems with Latent Diffusion Models}
\label{alg:resample}
\begin{algorithmic}
\Require Measurements $\bm{y}$, $\mathcal{A}(\cdot)$, Encoder $\mathcal{E}(\cdot)$, Decoder $\mathcal{D}(\cdot)$, Score function $\bm{s}_{\theta}(\cdot, t)$, Pretrained LDM Parameters $\beta_t$, $\bar{\alpha}_t$, $\eta$, $\delta$, Hyperparameter $\gamma$ to control $\sigma^2_t$, Time steps to perform resample $C$
\State{$\bm{z}_T \sim \mathcal{N}(\bm{0}, \bm{I})$}
\Comment{Initial noise vector}
\For{$t=T-1, \ldots, 0$}
\State $\pmb{\epsilon}_1 \sim \mathcal{N}(\bm{0}, \bm{I})$
\State $\hat{\bm{\epsilon}}_{t+1} = \bm{s}_{\theta}(\bm{z}_{t+1}, {t+1})$
\Comment{Compute the score}
\State $\hat{\bm{z}}_0(\bm{z}_{t+1}) = \frac{1}{\sqrt{\bar{\alpha}_{t+1}}} (\bm{z}_{t+1} - \sqrt{1-\bar{\alpha}_{t+1}}\hat{\bm{\epsilon}}_{t+1})$
\Comment{Predict $\hat{\bm{z}}_0$ using Tweedie's formula}
\State $\bm{z}'_{t} = \sqrt{\bar{\alpha}_{t}}\hat{\bm{z}}_0(\bm{z}_{t+1}) + \sqrt{1 - \bar{\alpha}_{t} - \eta\delta^2} \hat{\bm{\epsilon}}_{t+1} + \eta\delta \pmb{\epsilon}_1 $
\Comment{Unconditional DDIM step}
% \State $\bm{z}'_{t} = \bm{z}'_{t} - \frac{\bar{\alpha}_t}{2} \nabla_{\bm{z}_t} \|\bm{y} - \mathcal{A}  (\mathcal{D}(\hat{\bm{z}}_0(\bm{z}_t))) \|_2^2$
% \Comment{(Optional) Latent-DPS step\footnotemark}
\If{$t \in C$}
\Comment{ReSample time step}
% \For{$i = k, \ldots, 1$}
%\State $\pmb{\epsilon}_2 \sim \mathcal{N}(\bm{0}, \bm{I})$
% \State $\bm{z}'_{t-k} = \text{TimeTravel}(\bm{z}'_{t} )$
%\State \smk{$\bm{z}'_{t-i} = \sqrt{\bar{\alpha}_{t-i}}\hat{\bm{z}}_0 + \sqrt{1 - \bar{\alpha}_{t-i} - \eta_{t-i+1}^2} \bm{s}_{\theta}(\bm{z}_{t-i+1}, t-i+1) + \eta_{t-i+1} \pmb{\epsilon}_2 $}
% \Comment{Reverse sample $k$ times}
% \State $\hat{\bm{z}}_{0}(\bm{z}_{t}) = \frac{1}{\sqrt{\bar{\alpha}_{t}}}(\bm{z}'_{t} -+ \sqrt{(1-\bar{\alpha}_{t})}\bm{s}_{\theta}(\bm{z}'_{t}, t))$\Comment{Use Tweedie's formula}
\State $\hat{\bm{z}}_0(\bm{y}) \in \underset{\bm{z}}{\argmin} \, \frac{1}{2}\|\bm{y} - \mathcal{A}(\mathcal{D}(\bm{z}))\|_2^2$
\Comment{Solve with initial point $\hat{\bm{z}}_{0}(\bm{z}_{t+1})$}
\State $\bm{z}_{t} = \text{StochasticResample}(\hat{\bm{z}}_0(\bm{y}), \bm{z}'_{t}, \gamma)$
\Comment{Map back to $t$}
\Else{}
\State{$\bm{z}_{t} = \bm{z}'_{t}$}
\Comment{Unconditional sampling if not resampling}
\EndIf
\EndFor
\State{ $\bm{x}_0 = \mathcal{D}(\bm{z}_0)$}
\Comment{Output reconstructed image}
\end{algorithmic}
\end{algorithm}
% \vspace{-20pt}

% \footnotetext{We observe that an additional Latent-DPS step can (sometimes) marginally increase the overall performance. We perform an ablation study on the performance of including Latent-DPS in the Appendix.}


\paragraph{Remapping Back to $\bm{z}_t$.}
\label{sec:resample_technique}
Following the flowchart in Figure~\ref{fig:resample_flowchart}, the next step is to map the measurement-consistent sample $\hat{\bm{z}}_0(\bm{y})$ back onto the data manifold defined by the noisy samples at time $t$ to continue the reverse sampling process. Doing so would be equivalent to computing the posterior distribution $p(\bm{z}_{t} | \bm{y})$.
%It is difficult to directly sample from $p(\bm{z_{t}} | \bm{y})$.
To incorporate $\hat{\bm{z}}_0(\bm{y})$ into the posterior, we propose to construct an auxiliary distribution $p(\hat{\bm{z}}_{t} | \hat{\bm{z}}_0(\bm{y}), \bm{y}) $ in replace of $p(\bm{z}_{t} | \bm{y})$. Here, $\hat{\bm{z}}_t$ denotes the remapped sample and $\bm{z}'_t$ denotes the unconditional sample before remapping. One simple way of computing this distribution to obtain $\hat{\bm{z}}_t$ is shown in Proposition~\ref{prop:stochastic_enc}.
%Intuitively, $\bm{\hat{z}}_{t}$ should contain information of both $\bm{z_{t}}$ and $\bm{y}$. We denote $p(\hat{\bm{z}}_t)$ be the distribution of the remapped sample and $p(\bm{z}'_t)$ be that of the original sample.
\begin{proposition}[Stochastic Encoding]
\label{prop:stochastic_enc}
%For sampling $\bm{\hat{z}}_{t}$ given $\hat{\bm{z}}_0(\bm{y})$ and $\bm{y}$, it is conditionally independent of $\bm{y}$. So we can use a simple Gaussian distribution to sample $\bm{\hat{z}}_{t}$
Since the sample $\hat{\bm{z}}_t$ given $\hat{\bm{z}}_0(\bm{y})$ and measurement $\bm{y}$ is conditionally independent of $\bm{y}$, we have that
    \begin{align}
        p(\hat{\bm{z}}_{t} |  \hat{\bm{z}}_0(\bm{y}), \bm{y}) = p(\hat{\bm{z}}_{t} |  \hat{\bm{z}}_0(\bm{y})) = \mathcal{N}(\sqrt{\bar{\alpha}_t} \hat{\bm{z}}_0(\bm{y}), (1 -\bar{\alpha}_{t})\bm{I}).
    \end{align}
\end{proposition}
We defer all of the proofs to the Appendix. 
Proposition~\ref{prop:stochastic_enc} provides us a way of computing $\hat{\bm{z}}_t$, which we refer to as \emph{stochastic encoding}.
%However, this estimation has a high variance since going forward multiple steps has a much larger variance than going forward one step. 
However, we observe that using stochastic encoding can incur a high variance when $t$ is farther away from $t=0$, where the ground truth signal exists. This large variance can often lead to noisy image reconstructions.
To address this issue, we propose a posterior sampling technique that reduces the variance by additionally conditioning on $\bm{z}'_t$, the unconditional sample at time $t$.
%The idea is that we do not want the remapped sample to be far from the original sample at time $t$. Let $\bm{z}'_t$ be the original sample at time $t$.
Here, the intuition is that
by using information of $\bm{z}'_t$, we can get closer to the ground truth $\bm{z}_t$, which effectively reduces the variance. In Lemma~\ref{lem:resample}, under some mild assumptions, we show that this new distribution $p(\hat{\bm{z}}_t | \bm{z}'_t, \hat{\bm{z}}_0(\bm{y}), \bm{y})$ is a tractable Gaussian distribution.
\begin{proposition}[Stochastic Resampling]
\label{lem:resample}
    Suppose that $p(\bm{z}'_t| \hat{\bm{z}}_t, \hat{\bm{z}}_0(\bm{y}), \bm{y})$ is normally distributed such that  $p(\bm{z}'_t| \hat{\bm{z}}_t, \hat{\bm{z}}_0(\bm{y}), \bm{y}) = \mathcal{N}(\bm{ \mu }_t, \sigma_t^2)$. If we let $p(\hat{\bm{z}_t} | \hat{\bm{z}}_0(\bm{y}), \bm{y})$ be a prior for $\bm{\mu}_t$, then the posterior distribution $p(\hat{\bm{z}}_t | \bm{z}'_t, \hat{\bm{z}}_0(\bm{y}), \bm{y})$ is given by 
    \begin{align}
    p(\hat{\bm{z}}_t | \bm{z}'_t, \hat{\bm{z}}_0(\bm{y}), \bm{y}) = \mathcal{N}\left( \frac{ \sigma_{t}^2 \sqrt{\bar{\alpha}_t}\hat{\bm{z}}_0(\bm{y}) + (1-\bar{\alpha}_t)\bm{z}'_{t} }{ \sigma_{t}^2 + (1 - \bar{\alpha}_t) }, \frac{\sigma_{t}^2 (1-\bar{\alpha}_t)}{\sigma_{t}^2 + (1 - \bar{\alpha}_{t})}\bm{I}  \right).
\end{align} 
\end{proposition}

We refer to this new mapping technique as \emph{stochastic resampling}. Since we do not have access to $\sigma_t^2$, it serves as a hyperparameter that we tune in our algorithm. The choice of $\sigma_t^2$ plays a role of controlling the tradeoff between prior consistency and data consistency. If $\sigma_t^2 \to 0$, then we recover unconditional sampling, and if $\sigma_t^2 \to \infty$, we recover stochastic encoding. 
We observe that this new technique also has several desirable properties, for which we rigorously prove in the next section.



%%%%%%==================

\subsection{Theoretical Results}
\label{sec:theory}

In Section~\ref{sec:prop}, we discussed that stochastic resampling induces less variance than stochastic encoding. Here, we aim to rigorously prove the validity of this statement.

\begin{lemma}
\label{thm:smallvariance}
Let $\tilde{\bm{z}}_t$ and $\hat{\bm{z}}_t$ denote the stochastically encoded and resampled image of $\hat{\bm{z}}_0(\bm{y})$, respectively. If $\text{VAR}(\bm{z}'_t) > 0$, then we have that $\text{VAR}(\hat{\bm{z}}_t) < \text{VAR}(\tilde{\bm{z}}_t)$.
\end{lemma}

\begin{theorem}
\label{thm:unbias}
If ${\hat{\bm{z}}}_0(\bm{y})$ is measurement-consistent such that $\bm{y} = \mathcal{A}(\mathcal{D}({\hat{\bm{z}}}_0(\bm{y})))$, i.e. $\hat{\bm{z}}_0= \hat{\bm{z}}_0(\bm{z}_t) = \hat{\bm{z}}_0(\bm{y})$, then stochastic resample is unbiased such that $\mathbb{E}[\hat{\bm{z}}_t |  \bm{y}] = \mathbb{E}[\bm{z}'_t]$.
\end{theorem}

% \begin{proof}(Sketch)
% We have that $\mathbb{E}[\hat{\bm{z}}_t | \bm{y}] = \mathbb{E}_{\bm{z}'_t}[\mathbb{E}_{\bm{\hat{z}}_0}[\mathbb{E}_{\hat{\bm{z}}_t}[\hat{\bm{z}}_t | \bm{z}'_t, \hat{\bm{z}}_0, \bm{y}]]]$. By using Lemma~\ref{lem:resample} for $\mathbb{E}_{\hat{\bm{z}}_t}[\hat{\bm{z}}_t | \bm{z}'_t, \hat{\bm{z}}_0, \bm{y}]$, we have $\mathbb{E}_{\bm{z}'_t}[\mathbb{E}_{\hat{\bm{z}}_0}  [\sqrt{\bar{\alpha}_t} \bm{\hat{z}}_0 | \bm{z}'_t, \bm{y}]] = \mathbb{E}[\bm{z}'_t] - (1 - \bar{\alpha}_t)\mathbb{E}_{\bm{z}'_t}[\nabla \log p(\bm{z}'_{t})]$. By the chain rule, we have that $\mathbb{E}_{\bm{z}'_t}[\nabla \log p(\bm{z}'_{t})] = 0$, which gives the desired result.
% \end{proof}

These two results, Lemma~\ref{thm:smallvariance} and Theorem~\ref{thm:unbias}, prove the benefits of stochastic resampling. At a high-level, these proofs rely on the fact the posterior distributions of both stochastic encoding and resampling are Gaussian and compare their respective means and variances.
In the following result, we characterize the variance induced by stochastic resampling, and show that as $t \to 0$, the variance decreases, giving us a reconstructed image that is of better quality.

\begin{theorem}
\label{thm:z0variance}
 Let $\bm{z}_0$ denote a sample from the data distribution and $\bm{z}_t$ be a sample from the noisy perturbed distribution at time $t$. Then,
 \begin{align*}
     \text{Cov}(\bm{z}_0 | \bm{z}_t) = \frac{(1 - \bar{\alpha}_t)^2}{\bar{\alpha}_t}\nabla^2_{\bm{z}_t}\log p_{\bm{z}_t}(\bm{z}_t) + \frac{1 - \bar{\alpha}_t}{\bar{\alpha}_t}\bm{I}.
 \end{align*}
\end{theorem}
By Theorem~\ref{thm:z0variance}, noice that since as $\alpha_t$ is an increasing sequence that converges to 1 as $t$ decreases,
the variance between the ground truth $\bm{z}_0$ and the estimated $\hat{\bm{z}}_0$
decreases to 0 as $t \to 0$, assuming that
$\nabla^2_{\bm{z}_t}\log p_{\bm{z}_t}(\bm{z}_t) < \infty$.
% As a result, ReSample is able to pick up better quality estimates of $\hat{\bm{z}}_0$ as t decreases. 
%As a result, we incorporate both the data(measurement) consistency and prior consistency in our proposed ReSample algorithm.
%Lemma~\ref{thm:smallvariance} proves that we can both effectively reduce and control the variance of our measurement-consistent sample. 
Following our theory, we empirically show that stochastic resampling can reconstruct signals that are less noisy than stochastic encoding, as shown in the next section.\let\thefootnote\relax\footnotetext{*We have updated the baseline results for PSLD. More details are provided in the Appendix (Section~\ref{sec:psld_baseline}).}

==> ReSample_arixv417/text/background.tex <==
\section{Background}

\subsection{Diffusion Models}
\paragraph{Denoising Diffusion Probabilistic Models.} We first briefly review the basic fundamentals of diffusion models, namely the denoising diffusion probabilistic model (DDPM) formulation~\cite{ddpm}. Let $\bm{x}_0 \sim p_{\text{data}}(\bm{x})$ denote samples from the data distribution. Diffusion models start by progressively perturbing data to noise via Gaussian kernels, which can be written as the variance-preserving stochastic differential equation (VP-SDE)~\cite{song2021scorebased} of the form
\begin{align}
\label{eq:forward_sde}
    d\bm{x} = -\frac{\beta_t}{2}\bm{x}dt + \sqrt{\beta_t}d\bm{w},
\end{align}
where $\beta_t \in (0, 1)$ is the noise schedule that is a monotonically increasing sequence of $t$ and $\bm{w}$ is the standard Wiener process. This is generally defined such that we obtain the data distribution when $t=0$ and obtain a Gaussian distribution when $t=T$, i.e. $\bm{x}_T \sim \mathcal{N}(\bm{0}, \bm{I})$. The objective of diffusion models is to learn the corresponding reverse SDE of Equation~(\ref{eq:forward_sde}), which is of the form
\begin{align}
\label{eq:reverse_sde}
    d\bm{x} = \left[  -\frac{\beta_t}{2}\bm{x} - \beta_t \nabla_{\bm{x}_t} \log p(\bm{x}_t)\right]dt + \sqrt{\beta_t}d\bar{\bm{w}},
\end{align}
where $d\bar{\bm{w}}$ is the standard Wiener process running backward in time and $\nabla_{\bm{x}_t} \log p(\bm{x}_t)$ is the (Stein) score function. In practice, we approximate the score function using a neural network $\bm{s}_{\theta}$ parameterized by $\theta$, which can be trained via denoising score matching~\cite{vincent}:
\begin{align}
\label{eq:score_matching}
    \hat{\theta} = \underset{\theta}{\argmin} \, \mbb{E}\left[ \| \bm{s}_{\theta}(\bm{x}_t, t) - \nabla_{\bm{x}_t} \log p(\bm{x}_t | \bm{x}_0)\|_2^2 \right],
\end{align}
where $t$ is uniformly sampled from $[0, T]$ and the expectation is taken over $t$, $\bm{x}_t \sim p(\bm{x}_t | \bm{x}_0)$, and $\bm{x}_0 \sim p_{\text{data}}(\bm{x})$.
Once we have access to the parameterized score function $\bm{s}_{\theta}$, we can use it to approximate the reverse-time SDE and simulate it using numerical solvers (e.g. Euler-Maruyama). 

%These numerical solvers yield different discretizations, and one type of discretization yields the ancestral update steps
%\begin{align}
%    \bm{x}_{t-1} = \frac{1}{\sqrt{1-\beta_t}} \left( \bm{x}_t - \beta_t \bm{s}_{\theta}(\bm{x}_t, t) \right) + \sqrt{\beta_t}\bm{\epsilon}, \quad t=T, \ldots, 0,
%\end{align}
%where $\bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I})$. Thus, upon drawing an initial sample $\bm{x}_T \sim \mathcal{N}(\bm{0}, \bm{I})$, we can iteratively follow the step above to obtain $\bm{x}_0$.



%\begin{figure}[t!]
%\centering
%\includegraphics[width=1.0\textwidth]{figures/flowchart57.jpg}
%\caption{An overview of our method of enable data consistency of latent diffusion models by ReSample}
%\label{fig:cherrypick}
%\end{figure}




\begin{figure}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figures/resample_flowchart1.pdf}
\caption{\textbf{Overview of our \textit{ReSample} algorithm during the reverse sampling process conditioned on the data constraints from measurement.} The entire sampling process is conducted in the latent space upon passing the sample through the encoder. The proposed algorithm performs hard data consistency at some time steps $t$ via a skipped-step mechanism.}
\label{fig:resample_flowchart}
\vspace{-10pt}
\end{figure}

\paragraph{Denoising Diffusion Implicit Models.}
As the DDPM formulation is known to have a slow sampling process, Song et al.~\cite{ddim} proposed denoising diffusion implicit models (DDIMs) that defines the diffusion process as a non-Markovian process to remedy this~\cite{ddpm, ddim, song2023consistency, lu2022dpmsolver}.
This enables a faster sampling process with the sampling steps given by
\begin{align}
\label{eq:ddimbackward}
    \bm{x}_{t-1} = \sqrt{\bar{\alpha}_{t-1}}\hat{\bm{x}}_0(\bm{x}_t) + \sqrt{1 - \bar{\alpha}_{t-1} - \eta\delta_t^2 } \bm{s}_{\theta}(\bm{x}_t, t) + \eta\delta_t  \bm{\epsilon}, \quad t=T, \ldots, 0,
\end{align}
where $\alpha_t = 1 - \beta_t$,  $\bar{\alpha}_t = \prod_{i=1}^t \alpha_i$, $\bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{I})$, $\eta$ is the temperature parameter, $\delta_t$ controls the stochasticity of the update step, and $\hat{\bm{x}}_0(\bm{x}_t)$ denotes the predicted $\bm{x}_0$ from $\bm{x}_t$ which takes the form 
\begin{align}
\label{eq:x0_ddim}
\hat{\bm{x}}_0(\bm{x}_t) = \frac{1}{\sqrt{\bar{\alpha}_t}} (\bm{x}_t + \sqrt{1-\bar{\alpha}_t}\bm{s}_{\theta}(\bm{x}_t, t)),
\end{align}
which is an application of Tweedie's formula.
Here, $\bm{s}_{\theta}$ is usually trained using the epsilon-matching score objective~\cite{ddim}. We use DDIM as the backbone of our algorithm and show how we can leverage these update steps for solving inverse problems.

\subsection{Diffusion Models for Solving Inverse Problems}

\paragraph{Solving Inverse Problems with Diffusion Models.}
Given measurements $\bm{y} \in \R^m$ from some forward measurement operator $\mathcal{A}(\cdot)$, we can use diffusion models to solve inverse problems by replacing the score function in Equation~(\ref{eq:reverse_sde}) with the conditional score function $\nabla_{\bm{x}_t} \log p(\bm{x}_t | \bm{y})$. Then by Bayes rule, notice that we can write the conditional score as
\begin{align*}
    \nabla_{\bm{x}_t} \log p(\bm{x}_t | \bm{y}) = \nabla_{\bm{x}_t} \log p(\bm{x}_t) + \nabla_{\bm{x}_t} \log p(\bm{y} | \bm{x}_t).
\end{align*}
This results in the reverse SDE of the form
\begin{align*}
    d\bm{x} = \left[  -\frac{\beta_t}{2}\bm{x} - \beta_t ( \nabla_{\bm{x}_t} \log p(\bm{x}_t) + \nabla_{\bm{x}_t} \log p(\bm{y} | \bm{x}_t) )\right]dt + \sqrt{\beta_t}d\bar{\bm{w}}.
\end{align*}
In the literature, solving this reverse SDE is referred as \emph{posterior sampling}. However, the issue with posterior sampling is that there does not exist an analytical formulation for the likelihood term $\nabla_{\bm{x}_t} \log p(\bm{y} | \bm{x}_t)$. To resolve this, there exists two lines of work: (1) to resort to alternating projections onto the measurement subspace to avoid using the likelihood directly~\cite{mcg, ddrm, ddnm} and (2) to estimate the likelihood under some mild assumptions~\cite{dps, song2023PiGDM}. For example, Chung et al.~\cite{dps} proposed diffusion posterior sampling (DPS) that uses a Laplacian approximation of the likelihood, which results in the discrete update steps
\begin{align}
\label{eq:dps_updates}
    \bm{x}_{t-1} &= \sqrt{\bar{\alpha}_{t-1}}\hat{\bm{x}}_0(\bm{x}_t) + \sqrt{1 - \bar{\alpha}_{t-1} - \eta\delta_t^2 } \bm{s}_{\theta}(\bm{x}_t, t) + \eta\delta_t  \bm{\epsilon} \\
    \bm{x}_{t-1} &= \bm{x}'_{t-1} - \zeta \nabla_{\bm{x}_t} \|\bm{y} - \mathcal{A}(\hat{\bm{x}}_0(\bm{x}_t)) \|_2^2,
\end{align}
where $\zeta \in \R$ can be viewed as a tunable step-size.
However, as previously mentioned, these techniques have limited applicability for real-world problems as they are all built on the pixel space. 


\paragraph{Solving Inverse Problems with Latent Diffusion Models.}

The limited applicability of pixel-based diffusion models can be tackled by alternatively utilizing more efficient LDMs as generative priors.
The setup for LDMs is the following: given an image $\bm{x} \in \mbb{R}^n$, we have an encoder $\mathcal{E}: \mbb{R}^n \to \mbb{R}^k$ and a decoder $\mathcal{D}: \mbb{R}^k \to \mbb{R}^n$ where $k \ll n$.
Let $\bm{z} = \mathcal{E}(\bm{x}) \in \mbb{R}^k$ denote the embedded samples in the latent space. 
%Latent diffusion models operate within this latent space denoted by $\bm{z} \in \R^k$
%by passing all of the images in the pixel space through the encoder.
One way of incorporating LDMs to solve inverse problems would be to replace the update steps in Equation~(\ref{eq:dps_updates}) with
\begin{align}
\label{eq:latent_dps_updates}
    \bm{z}'_{t-1} &= \sqrt{\bar{\alpha}_{t-1}}\hat{\bm{z}}_0(\bm{z}_t) + \sqrt{1 - \bar{\alpha}_{t-1} - \eta \delta_t^2} \bm{s}_{\theta}(\bm{z}_t, t) + \eta\delta_t \bm{\epsilon}, \\
\label{eq:latent_dps_gradient}
    \bm{z}_{t-1} &= \bm{z}'_{t-1} - \zeta \nabla_{\bm{z}_t} \|\bm{y} - \mathcal{A}  (\mathcal{D}(\hat{\bm{z}}_0(\bm{z}_t))) \|_2^2,
\end{align}
After incorporating LDMs, this can be viewed as a non-linear inverse problem due to the non-linearity of the decoder $\mathcal{D}(\cdot)$. As this builds upon the idea behind DPS, we refer to this algorithm as \emph{Latent-DPS}.
While this formulation seems to work, we empirically observe that Latent-DPS often produces reconstructions that are often noisy or blurry and inconsistent with the measurements. We conjecture that since the forward operator involving the decoder is highly nonconvex, the gradient update may lead towards a local minimum. We provide more insights in Appendix (Section D).



% We conjecture that this occurs because there can exist infinitely many latents $\bm{z}_0 \in \R^k$ that correspond to the same set of measurements, and thus Equation~(\ref{eq:latent_dps_gradient}) can lead us towards a local minimum.



==> ReSample_arixv417/text/experiments.tex <==
\section{Experiments}
\label{sec:experiments}


\setlength{\tabcolsep}{5pt}
\begin{table}[t!]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lll|lll}
% \hline\noalign{\smallskip}
\hline
 \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Super Resolution $4\times$} & \multicolumn{3}{c}{Inpainting (Random $70\%$)} \\

& LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$  \\

\hline
DPS~\cite{dps} & $0.173\pm 0.04$ & $28.41 \pm 2.20$ & $0.782 \pm 0.06$ & $\underline{0.102} \pm 0.02$ & $\underline{32.48} \pm 2.30$ & $\underline{0.899} \pm 0.03$ \\
MCG~\cite{mcg}  & $0.193 \pm 0.03$ & $25.92 \pm 2.35$ & $0.740 \pm 0.05$ &$0.134 \pm 0.03$ & $29.53 \pm 2.70$ & $0.847 \pm 0.05$\\
ADMM-PnP~\cite{plugmri} & $0.304 \pm 0.04$ & $21.08 \pm 3.13$ & $0.631 \pm 0.11$   & $0.627 \pm 0.07$ & $15.40 \pm 2.09$ & $0.342 \pm 0.09$ \\
% \hhline{~-----}
% \hline
  DDRM~\cite{ddrm} & $0.151 \pm 0.03$   & $\underline{29.49} \pm 1.93$  & $0.817 \pm 0.05$ & $0.166 \pm 0.03$ & $27.69 \pm 1.54$& $0.798 \pm 0.04$\\

  DMPS~\cite{meng2022diffusion} & $\underline{0.147} \pm 0.03$ & $28.48 \pm 1.92$ & $\underline{0.811} \pm 0.05$ & $0.175 \pm 0.03$ & $28.84 \pm 1.65$  & $0.826 \pm 0.03$ \\
\hline
 Latent-DPS &  $0.272 \pm 0.05$& $26.83 \pm 2.00$  & $0.690 \pm 0.07$  & $0.226 \pm 0.04$ & $26.23 \pm 1.84$ & $0.703 \pm 0.07$\\
  PSLD-LDM$^*$~\cite{rout2023solving}  & $0.209 \pm 0.10$  & $27.61 \pm 2.95$  & $0.704 \pm 0.17$   &$0.260 \pm 0.08$ & $27.07 \pm 2.45$ & $0.689 \pm 0.11 $ \\
\hline

\hline
  ReSample (Ours) & $\bm{0.144} \pm 0.029$ & $\bm{30.45} \pm 2.09$  & $\bm{0.832} \pm 0.05$ & $\bm{0.082} \pm 0.02$ & $\bm{32.77} \pm 2.23$ & $\bm{0.903} \pm 0.03$\\
\hline
\end{tabular}}
\end{center}
% \vspace{-8pt}
\caption{\textbf{Quantitative results of super resolution and inpainting on the CelebA-HQ dataset.} Input images have an additive Gaussian noise with $\sigma_{\bm{y}} = 0.01$. Best results are in bold and second best results are underlined.}
\label{table:celeb1}
\vspace{-12pt}
\end{table}

\setlength{\tabcolsep}{5pt}
\begin{table}[t!]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lll|lll}
% \hline\noalign{\smallskip}
\hline
 \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Nonlinear Deblurring} & \multicolumn{3}{c}{Gaussian Deblurring}  \\

& LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\

\hline
 DPS~\cite{dps} & $0.230 \pm 0.065$ & $\underline{26.81} \pm 2.84$ & $\underline{0.720} \pm 0.077$ & $0.175 \pm 0.03$ &  $28.36 \pm 2.12$ & $0.772 \pm 0.07$  \\
% \hhline{~-----}
% \hline

  MCG~\cite{mcg}  &-& -& - & $0.517 \pm 0.06$&$15.85 \pm 1.08$& $0.536 \pm 0.08$ \\

  ADMM-PnP~\cite{plugmri} &$0.499 \pm 0.073$ & $16.17 \pm 4.01$& $0.359 \pm 0.140$ & $0.289 \pm 0.04$ & $20.98 \pm 4.51$  & $0.602 \pm 0.15$  \\

  DDRM~\cite{ddrm}  & - & -  & -  & $0.193 \pm 0.04$ & $26.88 \pm 1.96 $ & $0.747 \pm 0.07 $ \\

  DMPS~\cite{meng2022diffusion}  & - & -  & -  & $0.206 \pm 0.04$ & $26.45 \pm 1.83$ & $0.726 \pm 0.07$ \\

\hline
  Latent-DPS &  $\underline{0.225} \pm 0.04$& $26.18 \pm 1.73$  & $0.703 \pm 0.07$  & $0.205 \pm 0.04$ & $27.42 \pm 1.84$ & $0.729 \pm 0.07$ \\
  PSLD-LDM$^*$~\cite{rout2023solving}  & - & -  & -  & $0.323 \pm 0.09$ & $24.21 \pm 2.79$ & $0.548 \pm 0.12$ \\
\hline

\hline
  ReSample (Ours)  & $\bm{0.153} \pm 0.03$ & $\bm{30.18} \pm 2.21$  & $\bm{0.828} \pm 0.05$ & $\bm{0.148} \pm 0.04$ & $\bm{30.69} \pm 2.14$ & $\bm{0.832} \pm 0.05$ \\
\hline
\end{tabular}}
\end{center}
% \vspace{-8pt}
\caption{\textbf{Quantitative results of Gaussian and nonlinear deblurring on the CelebA-HQ dataset.} Input images have an additive Gaussian noise with $\sigma_{\bm{y}} = 0.01$. Best results are in bold and second best results are underlined. For nonlinear deblurring, some baselines are omitted, as they can only solve \emph{linear} inverse problems.}
\label{table:celeb2}
\vspace{-8pt}
\end{table}

We conduct experiments to solve both linear and nonlinear inverse problems on natural and medical images. We compare our algorithm to several state-of-the-art methods that directly use the pixel space: DPS~\cite{dps}, Manifold Constrained Gradients (MCG)~\cite{mcg}, Denoising Diffusion Destoration Models (DDRM)~\cite{ddrm}, Diffusion Model Posterior Sampling (DMPS)~\cite{meng2022diffusion}, 
and plug-and-play using ADMM (ADMM-PnP)~\cite{plugmri}. 
We also compare our algorithm to Latent-DPS and Posterior Sampling with Latent Diffusion (PSLD)~\cite{rout2023solving},
a concurrent work we recently notice also tackling latent diffusion models.
% \footnotemark\footnotetext{At the time of writing this paper, we were not aware of the work proposed by~\cite{fabian2023adapt}.}.
Various quantitative metrics are used for evaluation including Learned Perceptual Image Patch Similarity (LPIPS) distance, peak signal-to-noise-ratio (PSNR), and structural similarity index (SSIM).
Lastly, we conduct ablation study to compare the performance of stochastic encoding and our proposed stochastic resampling technique as mentioned in Section~\ref{sec:resample_technique}, and also demonstrate the memory efficiency gained by leveraging LDMs. \\
% We test our algorithm on both linear and nonlinear inverse problems on natural and medical images.
% For natural images we conducted experiments on FFHQ \cite{ffhq} and CelebA \cite{celeb}datasets. For medical images we tested sparse-view CT reconstruction on the AAPM \cite{ldct} dataset. We observe that ReSample achieves superior performance across a wide range of tasks. 
% We compare our algorithm to several state-of-the-art methods that directly use the pixel space –
% DPS [6], manifold constrained gradients (MCG) [9], and plug-and-play using ADMM (ADMMPnP) [43]. We also use Latent-DPS as a baseline to show the superiority of our algorithm in dealing
% with latent diffusion models. For quantitative comparison, we use several commonly used metrics:
% Learned Perceptual Image Patch Similarity (LPIPS) distance, peak signal-to-noise-ratio (PSNR),
% and structural similarity index (SSIM). an ablation study, we compare the performance of stochastic
% encoding and our proposed stochastic resampling as mentioned in Section 3. Lastly, we demonstrate
% the memory efficiency of our proposed algorithm gained by leveraging latent diffusion models.
% % 

\subsection{Experimental Results}
\paragraph{Experiments on Natural Images.} For the experiments on natural images, we use datasets FFHQ~\cite{ffhq}, CelebA-HQ~\cite{celeb}, and LSUN-Bedroom~\cite{lsun} with the image resolution of $256\times256\times3$. We take pre-trained latent diffusion models LDM-VQ4 trained on FFHQ and CelebA-HQ provided by Rombach et al.~\cite{stablediffusion} with autoencoders that yield images of size $64\times64\times3$, and DDPMs~\cite{ddpm} also trained on FFHQ and CelebA-HQ training sets. Then, we sample $100$ images from both the FFHQ and CelebA-HQ validation sets for testing evaluation. For computing quantitative results, all images are normalized to the range $[0, 1]$. All experiments had Gaussian measurement noise with standard deviation $\sigma_{\bm{y}} = 0.01$. Due to limited space, we put the results on FFHQ and details of the hyperparameters to the Appendix.

% that are also used by~\cite{dps} and~\cite{dhariwal2021diffusion}. 





%------------------------------------------

For linear inverse problems, we consider the following tasks: (1) Gaussian deblurring, (2) inpainting (with a random mask), and (3) super resolution. For Gaussian deblurring, we use a kernel with size $61 \times 61$ with standard deviation $3.0$. 
For super resolution, we use bicubic downsampling and a random mask with varying levels of missing pixels for inpainting. For nonlinear inverse problems, we consider nonlinear deblurring as proposed by Chung et al.~\cite{dps}.
The quantitative results are displayed in Tables~\ref{table:celeb1} and~\ref{table:celeb2}, with qualitative results in Figure~\ref{fig:linear_results}. In Tables~\ref{table:celeb1} and~\ref{table:celeb2},
we can see that ReSample significantly outperforms all of the baselines across all three metrics on the CelebA-HQ dataset. We also observe that ReSample performs better than or comparable to all baselines on the FFHQ dataset as shown in the Appendix.
Interestingly, we observe that PSLD~\cite{rout2023solving} seems to struggle in the presence of measurement noise, often resulting in reconstructions that underperform compared to pixel-based methods. Remarkably, our method excels in handling nonlinear inverse problems, further demonstrating the flexibility of our algorithm. We further demonstrate the superiority of ReSample for handling nonlinear inverse problems in Figure~\ref{fig:nonlinear_ablation}, where we show that we can consistently outperform DPS.




\begin{figure}[t!]
\centering
\includegraphics[width=1.0\textwidth]{figures/Natural_images.pdf}
\vspace{-12pt}
\caption{\textbf{Qualitative results of multiple tasks on the LSUN-Bedroom and CelebA-HQ datasets.} All inverse problems have Gaussian measurement noise with variance $\sigma_{\bm{y}} = 0.01$.}
\vspace{-8pt}
\label{fig:linear_results}
\end{figure}





% \textbf{Tasks}: 
% For linear inverse problems, we consider the following tasks: (1) Gaussian deblurring, (2) inpainting (with a random mask), and (3) super resolution. For Gaussian deblurring, we use a kernel with size $61 \times 61$ with standard deviation $3.0$. For super resolution, we use bicubic downsampling. Lastly, for inpainting, we use random masks with 70\% of missing pixels. 
% For nonlinear deblurring:  we leverage the neural network approximated forward model as in \cite{nonlinearblur}. For all tasks, we added a Gaussian noise with $\sigma_y = 0.01$ in the measurement domain.

% \textbf{Backbone models}:
% For LDM-based methods, we use LDM-VQ4 \cite{stablediffusion} trained on FFHQ \cite{ffhq}, and Celeba \cite{celeb}. We use the same pretrained model for Latent-DPS, PSLD, and ReSample.
% For pixel diffusion based methods, we use DDPM \cite{ddpm} trained on FFHQ \cite{ffhq}, and Celeba \cite{celeb} respectively. We use the same pretrained model for DPS, MCG, DDRM, and DMPS.
% For plug-and-play methods, we use DnCNNN denoiser provided by \cite{dncnn}. 
% \textbf{Baselines}:
% We consider two types of baselines: algorithms that solve inverse problems in the pixel space and those in the latent space. For pixel-space algorithms, we 
% \textbf{Backbone models}:  
% Backbone model: We use LDM-VQ4 \cite{stablediffusion} trained on FFHQ \cite{ffhq}, and Celeba \cite{celeb} for 


% \begin{wraptable}{r}{6.25cm}
% \caption{Results for nonlinear deblurring with $\sigma_{\bm{y}} = 0.05$.}
% \label{table:nonlinear_quant}
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{l|lll}
% % \hline\noalign{\smallskip}
% \hline
%  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Nonlinear Deblurring}\\
% %\hhline{~------}
% & LPIPS$\downarrow$& PSNR$\uparrow$ & SSIM$\uparrow$ \\
% \hline
% % \hline
%  Latent-DPS \cite{dps} & 0.351 & 22.39 & 0.560  \\


%  ADMM-PnP \cite{dps} & 0.424 & 21.82 & 0.489  \\
% % \hhline{~-----}
% % \hhline{~-----}
% % \hline
% DPS \cite{mcg} & \textbf{0.223} & 25.10 & 0.684 \\
% \hline
%   ReSample & 0.225 & \textbf{25.58}  & \textbf{0.710} \\
% \hline

% \end{tabular}}
% \end{wraptable} 



\begin{figure}[t!]
\centering
\includegraphics[width=0.775\textwidth]{figures/ReSample_CT_demo.jpeg}
\vspace{-8pt}
\caption{\textbf{Qualitative results of CT reconstruction on the LDCT dataset.} 
We annotate the critical image structures in a red box, and zoom in below the image.}
\label{fig:resample_Medical}
\vspace{-10pt}
\end{figure}


\setlength{\tabcolsep}{5pt}
\begin{table}[t!]
\begin{center}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l|ll|ll|ll}
% \hline\noalign{\smallskip}
\hline
 \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Abdominal} & \multicolumn{2}{c|}{Head} & \multicolumn{2}{c}{Chest}\\
%\hhline{~------}

& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

\hline
 Latent-DPS & 26.80 $\pm 1.09$ &  0.870 $\pm 0.026$ & 28.64 $\pm 5.38$& 0.893 $\pm 0.058$ & 25.67$\pm 1.14$  & 0.822 $\pm 0.033$\\
% \hhline{~-----}
% \hhline{~-----}
% \hline
MCG \cite{mcg} & 29.41 $\pm 3.14$& 0.857 $\pm 0.041$ & 28.28 $\pm 3.08$& 0.795 $\pm 0.116$ & 27.92 $\pm 2.48$ & 0.842 $\pm 0.036$\\

DPS~\cite{dps}  & 27.33 $\pm 2.68$& $0.715 \pm 0.031$ & 24.51 $\pm 2.77$ & 0.665 $\pm 0.058$ & 24.73 $\pm 1.84$ & 0.682 $\pm 0.113$\\
\hline
 PnP-UNet ~\cite{adaptive-inverse}& \underline{32.84} $\pm 1.29$&  \underline{0.942} $\pm 0.008$ & \underline{33.45} $\pm 3.25$ & \underline{0.945} $\pm 0.023$ & 29.67 $\pm 1.14$ & \underline{0.891} $\pm 0.011$\\

  FBP & 26.29 $\pm 1.24$& 0.727 $\pm 0.036$ & 26.71 $\pm 5.02$ & 0.725 $\pm 0.106$& 24.12 $\pm 1.14$& 0.655 $\pm 0.033$\\

 FBP-UNet \cite{unet} & 32.77 $\pm 1.21$ & 0.937 $\pm 0.013$& 31.95 $\pm 3.32$& 0.917 $\pm 0.048$ & \underline{29.78} $\pm 1.12$& 0.885 $\pm 0.016$\\
\hline
  ReSample (Ours) & \textbf{35.91} $\pm 1.22$ &  \textbf{0.965} $\pm 0.007$& \textbf{37.82} $\pm 5.31$ & \textbf{0.978} $\pm 0.014$ & \textbf{31.72} $\pm 0.912$& \textbf{0.922} $\pm 0.011$\\
\hline

\end{tabular}}
\end{center}
% \vspace{-8pt}
\caption{\textbf{Quantitative results of CT reconstruction on the LDCT dataset}. Best results are in bold and second best results are underlined.}
\label{table:ct_errorbar}
\vspace{-8pt}
\end{table}

\paragraph{Experiments on Medical Images.} 
For experiments on medical images, we fine-tune LDMs on 2000 2D computed tomography (CT) images with image resolution of $256\times256$, randomly sampled from the AAPM LDCT dataset~\cite{ldct} of 40 patients, and test on the 300 2D CT images from the remaining 10 patients. We take the FFHQ LDM-VQ4 model provided by Rombach et al.~\cite{stablediffusion} as pre-trained latent diffusion model in this experimental setting followed by 100K fine-tuning iterations. Then, we simulate CT measurements (sinograms) with a parallel-beam geometry using 25 projection angles equally distributed across 180 degrees using the~\texttt{torch-radon} package~\cite{torch_radon}. Following the natural images, the sinograms were perturbed with additive Gaussian measurement noise with $\sigma_{\bm{y}} = 0.01$. Along with the baselines used in the natural image experiments, we also compare to the following methods:
(1) Filtered Backprojection (FBP), which is a standard conventional CT reconstruction technique, and (2) FBP-UNet, a supervised learning method that maps the FBP reconstructed images to ground truth images using a UNet model.
For FBP-Unet and PnP-UNet, we trained a model on 3480 2D CT from the training set. For MCG and DPS, we used the pre-trained checkpoints provided by Chung et al.~\cite{mcg}. We present visual reconstructions with highlighted critical anatomic structures in Figure~\ref{fig:resample_Medical} and quantitative results in Table~\ref{table:ct_errorbar}. Here, we observe that our algorithm outperforms all of the baselines in terms of PSNR and SSIM. Visually, we also observe that our algorithm is able to reconstruct smoother images that have more accurate and sharper details. %Although MCG can also reconstruct similar sharp details, it often incurs a lot of noise, which may not be acceptable for more realistic medical imaging settings. 

\subsection{Ablation Studies}

\paragraph{Effectiveness of the Resampling Technique.}

Here, we validate our theoretical results by conducting ablation studies on stochastic resampling. Specifically, we perform experiments on the LSUN-Bedroom and CelebA-HQ datasets with tasks of Gaussian deblurring and super-resolution. As shown in Figure~\ref{fig:resampling_encoding}, we observe that stochastic resampling reconstructs smoother images with higher PSNRs compared to stochastic encoding, corroborating our theory.

\vspace{-6pt}
\paragraph{Effectiveness of Hard Data Consistency.} 
In Figure~\ref{fig:nonlinear_ablation}, we perform an ablation study on the ReSample frequency on CT reconstruction. This observation is in line with what we expect intuitively, as more ReSample time steps (i.e., more data consistency) lead to more accurate reconstructions.
More specifically, we observe in Figure~\ref{fig:nonlinear_ablation} (right) that if we perform more iterations of ReSample, we obtain reconstructions with higher PSNR.

\begin{wraptable}{r}{10cm}
\vspace{-14pt}
\caption{Memory Usage of Different Methods for Gaussian Deblurring on the FFHQ Dataset}
\vspace{-6pt}
\label{table:memory256}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{l | l|l | l | l}
\hline
Model & Algorithm & Model Only & Memory Increment & Total \\
\hline
DDPM & DPS & \textbf{1953MB} & +3416MB (175\%) & 5369MB \\
& MCG &  & +3421MB (175\%) & 5374MB \\
& DMPS &  & +5215MB (267 \%) & 7168MB \\
& DDRM & & +18833MB (964 \%) & 20786MB \\
\hline
LDM & PSLD & 3969MB & +5516MB (140\%) & 9485MB \\ 
& ReSample &  & \textbf{+1040MB (26.2\%)} & \textbf{5009MB}  \\
\hline
\end{tabular}}
\label{table:memory}
\end{wraptable}


\begin{figure}[t!]
\centering
\includegraphics[width=0.8\textwidth]{figures/Stochastic_Resample.pdf}
\caption{\textbf{Effectiveness of our resampling technique compared to stochastic encoding.} Results were demonstrated on the LSUN-Bedroom and CelebA-HQ datasets with measurement noise of $\sigma_{\bm{y}} = 0.05$ to highlight the effectiveness of stochastic resample.}
\vspace{-10pt}
\label{fig:resampling_encoding}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/nonlinear_ablation.pdf}
    \caption{\textbf{Additional results on the performance of ReSample.} Left: Results on nonlinear deblurring highlighting the performance of ReSample. Right: Ablation study on the ReSample frequency on the performance.}
    \label{fig:nonlinear_ablation}
\end{figure}

%\vspace{-6pt}
\paragraph{Memory Efficiency.}
To demonstrate the memory efficiency of our algorithm, we use the command \\\texttt{nvidia-smi} to monitor the memory consumption during solving an inverse problem, in comparison to our baselines. We present the memory usage for Gaussian deblurring on the FFHQ dataset in Table~\ref{table:memory}. Although the entire LDM models occupy more memory due to the autoencoders, our algorithm itself exhibits memory efficiency, resulting in lower overall memory usage. This underscores its potential in domains like medical imaging, where memory complexity plays a crucial role in feasibility.
% \bowen{\textbf{Ablation studies} in the Appendix further showcase the effectiveness of our ReSample module.

% \begin{figure}[t!]
% \includegraphics[width=0.4\textwidth]{figures/Timesteps_perf.png}
% \caption{CT reconstruction performance v.s. number of time steps to perform optimization/resample tested on 50 chest CT images. It shows performance increasing with more time steps but with additional computational cost.}
% \label{fig:resample_celeb_ablation}
% \end{figure}


% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.4\textwidth]{figures/hard_consistency_plot.png}
% \caption{Performance of different $\gamma$ values which control the strength of hard consistency for Gaussian Deblurring on 50 samples from Celeba validation dataset. Note that when $\gamma$ is very small, it is close to unconditional sampling}
% \label{fig:resample_celeb_ablation}
% \end{figure}
% \usepackage{subfigure}




% We study how the resample module improves the reconstruction performance. In Figure.~\ref{fig:timesteps}, we tested the CT reconstruction performance with increasing numbers of time steps to perform the hard optimization and the resample module. We observe that performance increases steadily when the number of time steps increases, which implies that the hard-consistency module is beneficial to reconstruction quality. \\
% \textbf{Computational Efficiency} since ReSample works with latent diffusion models, except the encoder-decoders, those models are memory-efficient. By design of our algorithm, after we obtain the uncondition sample from the diffusion model, we can free the memory of the diffusion model and only use the decoder to perform optimization, and then free the memory of the decoder to use the latent diffusion model again. As table.~\ref{table:memory256} demonstrates that even LDM combined with the autoencoder uses more memory than the DDPM, we can achieve the lowest memory across all algorithms. We observe more memory saving at higher resolution as shown in the Appendix. 

% \begin{wraptable}{r}{5cm}
% % \vspace{-14pt}
% \caption{Memory Usage of different algorithms with different pretrained models for Gaussian Deblurring on FFHQ dataset}
% \label{table:memory256}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l | l|l | l | l}
% \hline
% Pretrained Model & Algorithm & Model Only & Memory Increment & Total Memory \\
% \hline
% DDPM & DPS & \textbf{1953MB} & +3416MB (175\%) & 5369MB \\
% & MCG &  & +3421MB (175\%) & 5374MB \\
% & DMPS &  & +5215MB (267 \%) & 7168MB \\
% & DDRM & & +18833MB (964 \%) & 20786MB \\
% \hline

% LDM & PSLD & 3969MB & +5516MB (140\%) & 9485MB \\ 
% & ReSample (Ours) &  & \textbf{+1040MB (26.2\%)} & \textbf{5009MB}  \\
% \hline
% \end{tabular}}
% \vspace{-4pt}
% \end{wraptable}


% \begin{wraptable}{r}{5cm}
% \vspace{-14pt}
% \caption{Memory Usage of different algorithms with different pretrained models for Gaussian Deblurring on ImageNet $512 \times 512$ images}
% \label{table:finetune}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l | l|l | l | l}
% \hline
% Pretrained Model & Algorithm & Model Only & Memory Increment & Total Memory \\
% \hline
% DDPM & DPS & \textbf{4394MB} & +6637MB (151\%) & 11031MB \\
% & MCG &  & +6637MB (151\%) & 11031MB \\
% & DMPS &  & +8731MB (199 \%) & 13125MB \\
% & DDRM & & +4530MB (103 \%) & 8924MB \\
% \hline

% LDM & PSLD & 5669MB & +5516MB (97.3\%) & 11612MB \\ 
% & ReSample (Ours) &  & \textbf{+1322MB (30.1\%)} & \textbf{7002MB}  \\
% \hline
% \end{tabular}}
% \vspace{-4pt}
% \end{wraptable}







\begin{comment}
    \begin{figure}
     \centering
     \begin{subfigure}{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/nonlinear_deblur_plus.pdf}
         \caption{More examples of nonlinear deblurring.}
         \label{fig:more_nonlinear}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.38\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Timesteps_perf.png}
         \caption{Performance v.s. number of time steps to perform resample}
         \label{fig:resample_timestep}
     \end{subfigure}
     \caption{More experimental results of nonlinear inverse problems and ablation study.}
     \vspace{-12pt}
     \label{fig:finalmaterials}
\end{figure}
\end{comment}




% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.6\textwidth]{figures/nonlinear_deblur_plus.pdf}
% \caption{}
% \label{fig:more_nonlinear}
% \end{figure}


\section{Conclusion}

In this paper, we propose \textit{ReSample}, an algorithm that can effectively leverage LDMs to solve \emph{general} inverse problems. We demonstrated that (1) our algorithm can reconstruct high-quality images compared to many baselines and (2) we can fine-tune existing models for medical imaging tasks and achieve an additional reduction in memory usage. One fundamental limitation of our method lies in the computational overhead of hard data consistency, which we leave as a significant challenge for future work to address and improve upon.

\section{Acknowledgement}
BS and LS acknowledges support from U-M MIDAS PODS Grant and U-M MICDE Catalyst Grant, and computing resource support from NSF ACCESS Program and Google Cloud Research Credits Program. This work used NCSA Delta GPU through allocation CIS230133 and ELE230011 from the Advanced Cyberinfrastructure Coordination Ecosystem: Services \& Support (ACCESS) program, which is supported by National Science Foundation grants \#2138259, \#2138286, \#2138307, \#2137603, and \#2138296. SMK and QQ acknowledge support from U-M START \& PODS grants, NSF CAREER CCF-2143904, NSF CCF-2212066, NSF CCF-2212326, ONR N00014-22-1-2529, AWS AI Award, and a gift grant from KLA.

==> ReSample_arixv417/text/introduction.tex <==
\section{Introduction}

Inverse problems arise from a wide range of applications across many domains, including computational imaging~\cite{inverse1, inverse2}, medical imaging~\cite{medicalimaging, medicalimaging2}, and remote sensing~\cite{angle, yolov5}, to name a few. When solving these inverse problems, the goal is to reconstruct an unknown signal $\bm{x}_* \in \R^n$ given observed measurements $\bm{y} \in \R^m$ of the form
$$
    \bm{y} = \mathcal{A}(\bm{x}_*) + \bm{\bm{\eta}},
$$
where $\mathcal{A}(\cdot):\R^n \to \R^m$ denotes some forward measurement operator (can be linear or nonlinear) and $\bm{\eta} \in \R^m$ is additive noise. Usually, we are interested in the case when $m < n$, which follows many real-world scenarios. When $m < n$, the problem is ill-posed and some kind of regularizer (or prior) is necessary to obtain a meaningful solution.


In the literature, the traditional approach of using hand-crafted priors (e.g. sparsity) is slowly being replaced by rich, learned priors such as deep generative models. Recently, there has been a lot of interests in using diffusion models as structural priors due to their state-of-the-art performance in image generation~\cite{beatgan, karras2022elucidating, song2023consistency}.
Compared to GANs, diffusion models are generally easier and more stable to train as they do not rely on an adversarial training scheme, making them a generative prior that is more readily accessible~\cite{beatgan}.
The most common approach for using diffusion models as priors is to resort to posterior sampling, which has been extensively explored in the literature~\cite{score, dps, mcg, ddrm, song2023PiGDM, chung2023fast, meng2022diffusion, denoisingself}. However, despite their remarkable success, these techniques exhibit several limitations. 
The primary challenge is that the majority of existing works that employ diffusion models as priors train these models directly in the pixel space, which requires substantial computational resources and a large volume of training data. In real-world applications such as computed tomography (CT) and magnetic resonance imaging (MRI) reconstruction, where images are inherently either 3D or even 4D~\cite{sparsemri}, training diffusion models directly in the pixel space is often infeasible.
%Secondly, diffusion models are known to suffer from slow sampling speeds as the reverse process is an iterative procedure. 
%Leveraging these models for inverse problem solving often requires a huge additional overhead, making them impractical for applications that need fast inference~\cite{stablediffusion, ddim, ddpm}. 


Latent diffusion models (LDMs), which embed data in order to operate in a lower-dimensional space, present a potential solution to this challenge, along with considerable improvements in computational efficiency~\cite{stablediffusion, latent2} by training diffusion models in a compressed latent space. They can also provide a great amount of flexibility, as they can enable one to transfer and generalize these models to different domains by fine-tuning on small amounts of training data~\cite{dreambooth}. 
Nevertheless, using LDMs to solve inverse problems poses a significant challenge.
The main difficulty arises from the 
inherent nonlinearity and nonconvexity of the decoder, making it challenging to directly apply existing solvers designed for pixel space. 
To address this issue, a concurrent work by Rout et al.~\cite{rout2023solving} recently introduced a posterior sampling algorithm operating in the latent space (PSLD), designed to solve \emph{linear} inverse problems with provable guarantees. However, we observe that PSLD may reconstruct images with artifacts in the presence of measurement noise.
% limiting its applicability in domains where accurate inference is crucial. 
Therefore, developing an efficient algorithm capable of addressing these challenges remains an open research question. 


%We empirically observe that this is mainly because data consistency is hard to guarantee through the non-linearity of latent priors coming from the encoder and decoder.
\begin{figure}[t!]
\centering
\includegraphics[width=1.0\textwidth]{figures/motivation.pdf}
\vspace{-10pt}
\caption{\textbf{Example reconstructions of our algorithm (\textit{ReSample}) on two noisy inverse problems, nonlinear deblurring and CT reconstruction, on natural and medical images, respectively.}}
\vspace{-10pt}
\label{fig:resample_examples}
\end{figure}



In this work, we introduce a novel algorithm named \textit{ReSample}, which effectively employs LDMs as priors for solving inverse problems. Our algorithm can be viewed as a two-stage process that incorporates data consistency by (1) solving a hard-constrained optimization problem, ensuring we obtain the correct latent variable that is consistent with the observed measurements, and (2) employing a carefully designed resampling scheme to map the measurement-consistent sample back onto the correct noisy data manifold. 
As a result, we show that our algorithm can achieve state-of-the-art performance on various inverse problem tasks and different datasets, compared to existing algorithms. Notably, owing to using the latent diffusion models as generative priors, our algorithm achieves improved computational efficiency with a reduction in memory complexity.
Below, we highlight some of our key contributions.
\begin{itemize}[leftmargin=*]




    % \item \textbf{Novel Methodology.}
    % We propose a novel algorithm that involves solving an optimization problem for data consistency, which we term \emph{hard data consistency}. Upon performing hard data consistency, we devise a resampling scheme that maps the measurement-consistent samples back onto the noisy data manifold to continue the reverse process.
    % To demonstrate the effectiveness of our algorithm, we show both theoretically and empirically that we can reconstruct samples that are consistent with both the LDM prior and measurements. Additionally, our method is flexible in the sense that it can be readily adapted to solve various inverse problems (\emph{both linear and nonlinear}) in a zero-shot manner.
    
    % % \item \textbf{Hard Data Consistency.} To ensure data consistency, we solve an optimization problem in the reverse process, a concept we term as \emph{hard data consistency}.
    % % Compared to existing techniques, hard data consistency allows us to solve both linear and nonlinear inverse problems with latent diffusion models. Since this method does not assume any fixed forward operator, it can be readily adapted to solve a wide range of problems given a pre-trained model.

    % % \Comment{tone down theoretical contribution}
    % % \item \textbf{Theoretical Contributions.} \textbf{\color{red} Throw this in the bullet above} Upon performing hard data consistency, we devise a novel scheme to project the measurement-consistent sample back onto the noisy data manifold to continue the reverse process. We rigorously show that our resampling method enjoys several beneficial properties such as unbiasedness and low variance.
    % \item \textbf{Reconstruction Quality and Memory Efficiency.} 
    % We achieve state-of-the-art performance on a variety of linear and nonlinear inverse problems: CT reconstruction, nonlinear deblurring, inpainting, and super resolution. Remarkably, our algorithm demonstrates exceptional proficiency in handling nonlinear inverse problems -- a distinctive feature, as existing solutions employing LDMs cannot handle such problems.
    % We also demonstrate a reduction in memory complexity when using LDMs, as well as the capability to fine-tune them with small datasets. This fine-tuning ability holds substantial implications in domains such as medical imaging, where data is frequently limited and scarce.

     
     %Furthermore, we demonstrate we are able to achieve satisfying performance by using LDMs fine-tuned on small medical dataset.
     
    
    % By using latent diffusion models, we show that one can fine-tune pre-trained models to generalize to different domains with a minimal amount of data samples.
    %\item \textbf{Memory efficiency.} Our approach demonstrates the potential of reducing computational costs by showing that solving inverse problems using latent diffusion models can save required GPU memory compared to approaches using pixel-space diffusion models. 

    \item We propose a novel algorithm that enables us to leverage latent diffusion models for solving general inverse problems (linear and nonlinear) through hard data consistency. 
    
    
    % \footnote{\small{To our best knowledge, we are the first to propose an algorithm that can tackle general (including nonlinear) inverse problems with latent diffusion models. Although there are concurrent work tacking a similar problem, these methods are restricted to linear problems \cite{rout2023solving}.}}
    
    \item Particularly, we carefully design a stochastic resampling scheme that can reliably map the measurement-consistent samples back onto the noisy data manifold to continue the reverse sampling process. We provide a theoretical analysis to further demonstrate the superiority of the proposed stochastic resampling technique.
    
    % To demonstrate the effectiveness of our algorithm, we show both theoretically and empirically that we can reconstruct samples that are consistent with both the LDM prior and measurements. Additionally, our method is flexible in the sense that it can be readily adapted to solve various inverse problems (\emph{both linear and nonlinear}) in a zero-shot manner.

    \item With extensive experiments on multiple tasks and various datasets, encompassing both natural and medical images, our proposed algorithm achieves state-of-the-art performance on a variety of linear and nonlinear inverse problems.
    % CT reconstruction, nonlinear deblurring, inpainting, and super resolution. 
    % Remarkably, our algorithm demonstrates exceptional proficiency in handling nonlinear inverse problems -- a distinctive feature, as existing solutions employing LDMs cannot handle such problems.
    % We also demonstrate a reduction in memory complexity when using LDMs, as well as the capability to fine-tune them with small datasets. 
    % This fine-tuning ability holds substantial implications in domains such as medical imaging, where data is frequently limited and scarce.
    
\end{itemize}



==> ReSample_arixv417/text/methods.tex <==



% Our main objective is to explore how we can leverage latent diffusion models~\cite{stablediffusion} to solve inverse problems. 
% Here, we assume that we have access to a well-trained latent diffusion model that sufficiently captures the data distribution of the target problem. 
% The setup for latent diffusion models is the following: given an image $\mbf{x} \in \mbb{R}^n$, we have an encoder $\mathcal{E}: \mbb{R}^n \to \mbb{R}^k$ and a decoder $\mathcal{D}: \mbb{R}^k \to \mbb{R}^n$ where $k \ll n$.
% Let $\mbf{z} = \mathcal{E}(\mbf{x}) \in \mbb{R}^k$ denote the embedding samples in the latent space. Latent diffusion models operate in this latent space by passing all of the images in the pixel space through this encoder to obtain embeddings. Similarly, the score function is also trained by replacing $\mbf{x} \in \mbb{R}^n$ with $\mbf{z} \in \mbb{R}^k$ in Equation~(\ref{eq:score_matching}). Upon using any sampling technique (e.g. DDIM or DDPM) to obtain ${\mbf{z}}_0$, the ``denoised'' latent embedding at $t=0$, one can compute ${\mbf{x}}_0 = \mathcal{D}({\mbf{z}}_0)$ to generate a synthetic image through the decoder.

% To solve inverse problems using latent diffusion models, notice that one possible method is to replace the update steps in Equation~(\ref{eq:dps_updates}) with
% \begin{align}
% \label{eq:latent_dps_updates}
%     \mbf{z}'_{t-1} &= \sqrt{\bar{\alpha}_{t-1}}\hat{\mbf{z}}_0(\mbf{z}_t) + \sqrt{1 - \bar{\alpha}_{t-1} - \eta \delta_t^2} \mbf{s}_{\theta}(\mbf{z}_t, t) + \eta\delta_t \pmb{\epsilon} \\
% \label{eq:latent_dps_gradient}
%     \mbf{z}_{t-1} &= \mbf{z}'_{t-1} - \zeta \nabla_{\mathbf{z}_t} \|\mathbf{y} - \mathcal{A}  (\mathcal{D}(\hat{\mathbf{z}}_0(\mathbf{z}_t))) \|_2^2,
% \end{align}
% which can be viewed as a non-linear inverse problem due to the non-linearity of the decoder $\mathcal{D}(\cdot)$. As this builds upon the idea behind DPS~\cite{dps}, we refer to this algorithm as Latent-DPS. However, we empirically observe that Latent-DPS often reconstructs signals that are noisy. We hypothesize that this occurs for three reasons: (1) during the early stages of sampling, the estimation of $\hat{\mbf{z}}_0(\mbf{z}_t)$ can have high variance, resulting in a gradient that points to a direction inconsistent with the measurements, (2) due to the non-convex nature of $\mathcal{D}(\cdot)$, the gradient update in Equation~(\ref{eq:latent_dps_gradient}) can push you towards a local minima~\cite{csgm}, and (3) DPS steps were derived using a locally linear manifold assumption, which the latent decoder violates. These issues can clash during the sampling stage, resulting in inaccurate (or noisy) reconstructions. We provide more intuition about these reasons in the Appendix.


% The key to the success of our method is more accurately estimating $\hat{\mbf{z}}_0(\mbf{z}_t)$, which essentially solve the issues raised by Latent-DPS.
% This type of data consistency is what we refer to as \textbf{hard data consistency}.
% Upon obtaining $\hat{\mbf{z}}_0(\mbf{y})$, we develop a novel scheme to project $\hat{\mbf{z}}_0(\mbf{y})$ back to the data manifold defined by the samples $\mbf{z}_t$ for continuing the reverse process of latent diffusion models. Our algorithm is outlined in Figure~\ref{fig:resample_flowchart} and Algorithm~\ref{alg:resample}.
% %\bowen{With trained perceptual compression autoencoder models, we are able to abstract away inperceptible, high-frequency details with an emphasis on semantic information of data \cite{stablediffusion}. Let $D$ be the pretrained decoder, and $\mathcal{E}$ be the pretrained encoder. $z_0$ can be sampled from $p_{x}(\mathcal{E}(x))$, and $z_t$ be sampled by the tractable Gaussian distribution $p(z_t| z_0)$. Then, the latent diffusion is trained by the following objective
% %\begin{align}
% %    L_{ldm} := \mbb{E}_{\mathcal{E}(x_0), \epsilon \in N(0,1), t}\left[ \| \mbf{\epsilon}(\mbf{x}_t, t) - \epsilon \| \right ],
% %\end{align}. When sampling we can firstly sample $z_0$ and then compute $x = D(z_0)$. }

% \begin{algorithm}[t]
% \caption{\texttt{ReSample}}
% \label{alg:resample}
% \begin{algorithmic}
% \Require Measurements $\mathbf{y}$, $\mathcal{A}(\cdot)$, Encoder $\mathcal{E}(\cdot)$, Decoder $\mathcal{D}(\cdot)$, Score function $s_{\theta}(\cdot, t)$, Parameters $\beta_t$, $\bar{\alpha}_t$, $\eta$, $\delta$, $\lambda$, Time steps for data consistency $C = \{1, \ldots, T\}$, Time travel iterations $k$
% \State{$\mbf{x}_T \sim \mathcal{N}(\mbf{0}, \mbf{I})$; $\mbf{z}_T = \mathcal{E}(\mbf{x}_T)$}
% \Comment{Initial noise vector}
% \For{$t=T-1, \ldots, 0$}
% \State $\pmb{\epsilon}_1 \sim \mathcal{N}(\mbf{0}, \mbf{I})$
% \State $\hat{\mbf{z}}_0 = \frac{1}{\sqrt{\bar{\alpha}_{t+1}}} (\mbf{z}_{t+1} - \sqrt{1-\bar{\alpha}_{t+1}}\mbf{s}_{\theta}(\mbf{z}_{t+1}, {t+1}))$
% \Comment{Predict $\hat{\mbf{z}}_0$}
% \State $\mbf{z}'_{t} = \sqrt{\bar{\alpha}_{t}}\hat{\mbf{z}}_0 + \sqrt{1 - \bar{\alpha}_{t} - \eta\delta^2} \mbf{s}_{\theta}(\mbf{z}_{t+1}, {t+1}) + \eta\delta \pmb{\epsilon}_1 $
% \Comment{Unconditional DDIM step}
% \If{$t \in C$}
% % \For{$i = k, \ldots, 1$}
% %\State $\pmb{\epsilon}_2 \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$
% \State $\mbf{z}'_{t-k} = \text{TimeTravel}(\mbf{z}'_{t} )$
% %\State \smk{$\mbf{z}'_{t-i} = \sqrt{\bar{\alpha}_{t-i}}\hat{\mbf{z}}_0 + \sqrt{1 - \bar{\alpha}_{t-i} - \eta_{t-i+1}^2} \mbf{s}_{\theta}(\mbf{z}_{t-i+1}, t-i+1) + \eta_{t-i+1} \pmb{\epsilon}_2 $}
% \Comment{Reverse sample $k$ times}
% \State $\hat{\mbf{z}}_{0}(\mbf{z}_{t}) = \frac{1}{\sqrt{\bar{\alpha}_{t-k}}}(\mbf{z}'_{t-k} + (1-\bar{\alpha}_{t-k})s_{\theta}(\mbf{z}'_{t-k}, t-k))$\Comment{Use Tweedie's formula}
% \State $\hat{\mbf{z}}_0(\mbf{y}) = \underset{\mbf{z}}{\argmin} \, \frac{1}{2}\|\mathbf{y} - \mathcal{A}(\mathcal{D}(\mathbf{z}))\|_2^2 + \frac{\lambda}{2}\|\mathbf{z} - \hat{\mathbf{z}}_0(\mbf{z}_{t})\|_2^2$
% \State $\mbf{z}_{t} = \text{StochasticResample}(\hat{\mbf{z}}_0(\mbf{y}), \mbf{z}'_{t})$
% \Comment{Map back to $t$}
% \Else{}
% \State{$\mbf{z}_{t} = \mbf{z}'_{t}$}
% \Comment{Unconditional sampling if no data consistency}
% \EndIf
% \EndFor
% \State{ $\mbf{x}_0 = \mathcal{D}(\mbf{z}_0)$}
% \end{algorithmic}
% \end{algorithm}

% \paragraph{Estimating $\hat{\mbf{z}}_0(\mbf{z}_t)$.}

% Following the flowchart in Figure~\ref{fig:resample_flowchart}, the first step is to estimate $\hat{\mbf{z}}_0(\mbf{z}_t)$. We want $\hat{\mbf{z}}_0(\mbf{z}_t)$ to have low variance and lie (closely) within the manifold of the real data distribution $p_{\text{data}}(\mbf{z})$. If the estimation is far from $p_{\text{data}}(\mbf{z})$, then the solution of the optimization problem in Equation~(\ref{eq:latentinversion}) will steer far from the ground truth. 
% To achieve this, we propose to use Tweedie's formula upon using the time-travel technique~\cite{freedom, repaint}. More precisely, our estimate of $\hat{\mbf{z}}_0(\mbf{z}_t)$ at iteration $t$ becomes
% \begin{align}
%     \hat{\mbf{z}}_0(\mbf{z}_t) = \mbb{E}[\mbf{z}_0 | \mbf{z}_{t-k}] = \frac{1}{\sqrt{\bar{\alpha}_{t-k}}} (\mbf{z}_{t-k} - (1-\bar{\alpha}_{t-k})\nabla \log p(\mbf{z}_{t-k})),
% \end{align} 
% where $\mbf{z}_{t-k}$ is sampled from $\mbf{z}_t$ using the standard reverse process.
% The intuition here is that going back $k$ steps can give us an estimate of $\hat{\mbf{z}}_0$ that is closer to the ground truth as we get closer to $t=0$.
% Then, after obtaining the estimate $\hat{\mbf{z}}_0(\mbf{z}_t)$, we can solve the optimization problem for data consistency at time $t$ as described in the next section. We would like to point out that although time traveling may seem costly, it hardly adds any overhead as we operate in the latent space~\cite{stablediffusion}. %We discuss our choices of $k$ and provide ablation studies on its effect in the Appendix.



% \paragraph{Hard Data Consistency via Optimization.}
% Then, as shown in Figure~\ref{fig:resample_flowchart}, upon obtaining $\hat{\mbf{z}}_0(\mbf{z}_t)$, we need to optimize $\hat{\mbf{z}}_0(\mbf{z}_t)$ such that it is measurement-consistent using Equation~(\ref{eq:latentinversion}).  However, solving the problem on every reverse sampling iteration $t$ can be very costly. To deal with this, we first remark that when we are closer to $t=T$, our estimate $\hat{\mbf{z}}_0(\mbf{z}_t)$ can be far from the ground truth, as the samples at these time steps are mainly dominated by noise. In this regime, we observe that solving the optimization problem for data consistency gives very marginal benefits. Moreover, in the literature, existing works that incorporate conditional diffusion models state the existence of a three stage phenomenon \cite{freedom}, where it shows that data consistency is really only beneficial for the semantic and refinement stage (the latter two stages when it is closer to $t=0$) of the sampling process~\cite{freedom}.
% Follow this reasoning, we split $T$ into three sub-intervals and only perform the optimization in the latter two intervals. This would yield both computational efficiency and accurate estimates of $\hat{\mbf{z}}_0(\mbf{z}_t)$.

% Furthermore, even during these two intervals, we observe that we do not need to solve the optimization problem on every iteration $t$. Because of the continuity of the sampling process, after each data-consistency optimization step, the samples in the following steps can still remain similar semantic or structural information to some extent. Thus, we ``reinforce'' the data consistency constraint during the sampling process via a skipped-step mechanism. Empirically, we see that it is sufficient to perform this on every $10$ (or so) iterations of $t$. One can think of hard data consistency as guiding the sampling process towards the ground truth signal $\mbf{x}^*$ such that it is consistent with the given measurements.
% Lastly, in the presence of measurement noise, minimizing Equation~(\ref{eq:latentinversion}) to have zero loss can lead to overfitting the noise. To remedy this, we perform early stopping, where we only minimize up to a noise-level-based threshold $\tau$.
% We will discuss the choices of $\tau$ in the Appendix.

% %If the estimation has a high variance, when we resample back, we will not have the reverse sampling pointing to a consistent direction \cite{ddim, geometric}. Specifically, we want to balance between two terms $\mathbb{E}(z_0 | z_t)$ and a sample from $p(z_0 | z_t)$. 
% %We propose to apply a time-travel technique to balance the above two terms. The algorithm is straightforward: perform reverse sampling for k steps (i.e. sample from $p(z_{t_0 -k } | z_{t_0})$, and then compute $\hat{z_0}(z_{t_0}) = \mathbb{E}(z_0 | z_{t_0-k})$

% %For computing $\mathbb{E}(z_0 | z_{t_0-k})$, we apply Tweedie's formula, which gives us: 
% %\begin{align}
% %\mathbb{E}(z_0 | z_{t-k}) = \frac{z_t - (1-\alpha_t) %\nabla_{\mbf{z}_t}\log p(z_t)}{\sqrt{\alpha_t}}
% %\end{align}, and we replace the score value by the pretrained latent diffusion model prediction $\nabla_{\mbf{z}_t}\log p(z_t) \approx \epsilon_{\theta}(z_t, t)$



% \paragraph{Remapping Back to $\mbf{z}_t$.}
% \label{sec:resample_technique}
% Upon obtaining the measurement-consistent sample $\hat{\mbf{z}}_0(\mbf{y})$ via hard data consistency, we need to map this sample back to the data manifold to continue the reverse sampling process, as shown in Fig.~\ref{fig:resample_flowchart}. Doing so would be equivalent to computing the posterior distribution $p(\mbf{z}_{t} | \mbf{y})$.
% %It is difficult to directly sample from $p(\mbf{z_{t}} | \mbf{y})$.
% To incorporate $\hat{\mbf{z}}_0(\mbf{y})$ into the posterior, we propose to construct an auxiliary distribution $p(\hat{\mbf{z}}_{t} | \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) $ in replace of $p(\mbf{z}_{t} | \mbf{y})$. Here, $\hat{\mbf{z}}_t$ denotes the remapped sample and $\mbf{z}'_t$ denotes the unconditional sample before remapping. One simple way of computing this distribution to obtain $\hat{\mbf{z}}_t$ is shown in Proposition~\ref{prop:stochastic_enc}.
% %Intuitively, $\mbf{\hat{z}}_{t}$ should contain information of both $\mbf{z_{t}}$ and $\mbf{y}$. We denote $p(\hat{\mbf{z}}_t)$ be the distribution of the remapped sample and $p(\mbf{z}'_t)$ be that of the original sample.
% \begin{proposition}[Stochastic Encoding]
% \label{prop:stochastic_enc}
% %For sampling $\mbf{\hat{z}}_{t}$ given $\hat{\mbf{z}}_0(\mbf{y})$ and $\mbf{y}$, it is conditionally independent of $\mbf{y}$. So we can use a simple Gaussian distribution to sample $\mbf{\hat{z}}_{t}$
% Since the sample $\hat{\mbf{z}}_t$ given $\hat{\mbf{z}}_0(\mbf{y})$ and measurement $\mbf{y}$ is conditionally independent of $\mbf{y}$, we have that
%     \begin{align}
%         p(\hat{\mbf{z}}_{t} |  \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) = p(\hat{\mbf{z}}_{t} |  \hat{\mbf{z}}_0(\mbf{y})) = \mathcal{N}(\sqrt{\bar{\alpha}_t} \hat{\mbf{z}}_0(\mbf{y}), (1 -\bar{\alpha}_{t})\mbf{I}).
%     \end{align}
% \end{proposition}
% We defer all of the proofs to the Appendix. Proposition~\ref{prop:stochastic_enc} provides us a way of computing $\hat{\mbf{z}}_t$, which we refer to as \textbf{stochastic encoding}.
% %However, this estimation has a high variance since going forward multiple steps has a much larger variance than going forward one step. 
% However, we observed that using stochastic encoding can incur a high variance when $t$ is farther away from $t=0$, where the ground truth signal exists. This large variance can often lead to noisy image reconstructions.
% To address this issue, we propose a posterior sampling technique that reduces the variance by additionally conditioning on $\mbf{z}'_t$, the unconditional sample at time $t$.
% %The idea is that we do not want the remapped sample to be far from the original sample at time $t$. Let $\mbf{z}'_t$ be the original sample at time $t$.
% Here, the intuition is that
% by using information of $\mbf{z}'_t$, we can get closer to the ground truth $\mbf{z}_t$, which effectively reduces the variance. In Lemma~\ref{lem:resample}, under some mild assumptions, we show that this new distribution $p(\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is a tractable Gaussian distribution.
% \begin{proposition}[Stochastic Resampling]
% \label{lem:resample}
%     Suppose that $p(\mbf{z}'_t| \hat{\mbf{z}}_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is normally distributed such that  $p(\mbf{z}'_t| \hat{\mbf{z}}_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) = \mathcal{N}(\mathbf{ \mu }_t, \sigma_t^2)$. If we let $p(\hat{\mbf{z}_t} | \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ be a prior for $\mbf{\mu}_t$, then the posterior distribution $p(\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is given by 
%     \begin{align}
%     p(\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) = \mathcal{N}\left( \frac{ \sigma_{t}^2 \sqrt{\bar{\alpha}_t}\hat{\mbf{z}}_0(\mbf{y}) + (1-\bar{\alpha}_t)\mbf{z}'_{t} }{ \sigma_{t}^2 + (1 - \bar{\alpha}_t) }, \frac{\sigma_{t}^2 (1-\bar{\alpha}_t)}{\sigma_{t}^2 + (1 - \bar{\alpha}_{t})}\mbf{I}  \right).
% \end{align} 
% \end{proposition}

% %Instead of using $p(\hat{\mbf{z}}_t | \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$, we want to sample from the posterior distribution of it: $p(\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$, which contains the information of $\mbf{z}'_t$. Since $p(\hat{\mbf{z}}_t | \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is an estimation of the ground truth $\mbf{z}_t$ at time $t$, we can use that as the prior distribution of the parameters of $p(\mbf{z}'_t| \mbf{\hat{z}}_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$.
% \begin{comment}
% \begin{lemma}
% \label{lem:prior}
% For sampling $\mbf{\hat{z}}_{t}$ given $\hat{\mbf{z}}_0(\mbf{y})$ and $\mbf{y}$, it is conditionally independent of $\mbf{y}$. So we can use a simple Gaussian distribution to sample $\mbf{\hat{z}}_{t}$
%     \begin{align}
%         p(\mbf{\hat{z}}_{t} |  \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) = p(\mbf{\hat{z}}_{t} |  \hat{\mbf{z}}_0(\mbf{y})) = \mathcal{N}(\sqrt{\alpha_t} \hat{\mbf{z}}_0(\mbf{y}), 1 -\alpha_{t})
%     \end{align}
% \end{lemma}
% \end{comment}
% %Lemma.\ref{lem:prior} gives a simple way to get back to time $t$: $\mbf{\hat{z}}_{t} = \sqrt{\bar{\alpha}_{t}} \hat{\mbf{z}}_0(\mbf{y}) + \sqrt{1 - \bar{\alpha}_{t}}\pmb{\epsilon}$. This method is what we refer to as \textbf{stochastic encoding}. 
% \begin{comment}
% \begin{lemma}
%     \label{lem: resample}
%     Suppose that $p(\mbf{z}'_t| \mbf{\hat{z}}_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is normally distributed by $N(\mathbf{ \mu }_t, \sigma_t^2)$, let $p(\mbf{\hat{z}_t} | \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ be the prior for $\mbf{\mu}_t$, then the posterior distribution $p(\mbf{\hat{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y})$ is given by 
%     \begin{align}
%     p(\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0(\mbf{y}), \mbf{y}) = \mathcal{N}\left( \frac{ \sigma_{t}^2 \sqrt{\alpha_t}\hat{\mbf{z}}_0(\mbf{y}) + (1-\alpha_t)\mbf{z}'_{t} }{ \sigma_{t}^2 + (1 - \alpha_t) }, \frac{\sigma_{t}^2 (1-\alpha_t)}{\sigma_{t}^2 + (1 - \alpha_{t})}\mbf{I}  \right),
% \end{align} 
% \end{lemma}.
% \end{comment}
% We refer to this new mapping technique as \textbf{stochastic resampling}. Since we do not have access to $\sigma_t^2$, it serves as a hyperparameter that we tune in our algorithm. The choice of $\sigma_t^2$ plays a role of controlling the tradeoff between prior consistency and data consistency. If $\sigma_t^2 \to 0$, then we recover unconditional sampling, and if $\sigma_t^2 \to \infty$, we recover stochastic encoding. 
% We observe that this new technique also has several desirable properties, for which we rigorously prove.
% %Now we also observe some desirable properties of the stochastic sampling comparing to stochastic encoding. 
% \begin{theorem}
% \label{thm:unbias}
% If ${\hat{\mbf{z}}}_0(\mbf{y})$ is measurement-consistent such that $\mbf{y} = \mathcal{A}(\mathcal{D}({\hat{\mbf{z}}}_0(\mbf{y})))$, i.e. $\hat{\mbf{z}}_0= \hat{\mbf{z}}_0(\mbf{z}_t) = \hat{\mbf{z}}_0(\mbf{y})$, then stochastic resample is unbiased such that $\mathbb{E}[\hat{\mbf{z}}_t |  \mbf{y}] = \mathbb{E}[\mbf{z}'_t]$.
% \end{theorem}
% %\begin{proof}(Sketch)
% % $\mathbb{E}[\mbf{\hat{z_t}} | \mbf{y}] = \mathbb{E}_{\mbf{z}'_t}[\mathbb{E}_{\mbf{\hat{z}}_0}[\mathbb{E}_{\mbf{\hat{z}}_t}[\mbf{\hat{z_t}} | \mbf{z}'_t, \hat{\mbf{z}}_0, \mbf{y}]]]$, for $\mathbb{E}_{\mbf{\hat{z}}_t}[\mbf{\hat{z_t}} | \mbf{z}'_t, \hat{\mbf{z}}_0, \mbf{y}]$, we can plug in Lemma.\ref{lem: resample}, and then we have $\mathbb{E}_{\mbf{z}'_t}[\mathbb{E}_{\mbf{\hat{z}}_0}  [\sqrt{\alpha_t} \mbf{\hat{z}}_0 | \mbf{z}'_t, \mbf{y}]] = \mathbb{E}[\mbf{z}'_t] - (1 - \alpha_t)\mathbb{E}_{\mbf{z}'_t}[\nabla \log p(\mbf{z}'_{t})]$. By chain rule, we have $\mathbb{E}_{\mbf{z}'_t}[\nabla \log p(\mbf{z}'_{t})] = 0$
% %\end{proof} 
% \begin{proof}(Sketch)
% We have that $\mathbb{E}[\hat{\mbf{z}}_t | \mbf{y}] = \mathbb{E}_{\mbf{z}'_t}[\mathbb{E}_{\mbf{\hat{z}}_0}[\mathbb{E}_{\hat{\mbf{z}}_t}[\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0, \mbf{y}]]]$. By using Lemma~\ref{lem:resample} for $\mathbb{E}_{\hat{\mbf{z}}_t}[\hat{\mbf{z}}_t | \mbf{z}'_t, \hat{\mbf{z}}_0, \mbf{y}]$, we have $\mathbb{E}_{\mbf{z}'_t}[\mathbb{E}_{\hat{\mbf{z}}_0}  [\sqrt{\bar{\alpha}_t} \mbf{\hat{z}}_0 | \mbf{z}'_t, \mbf{y}]] = \mathbb{E}[\mbf{z}'_t] - (1 - \bar{\alpha}_t)\mathbb{E}_{\mbf{z}'_t}[\nabla \log p(\mbf{z}'_{t})]$. By the chain rule, we have that $\mathbb{E}_{\mbf{z}'_t}[\nabla \log p(\mbf{z}'_{t})] = 0$, which gives the desired result.
% \end{proof}
% %\begin{theorem}    
% %\label{lem:smallvariance}
% %If $\text{VAR}(\mbf{z}'_t) > 0$, then the variance of stochastic resampling is smaller than that of stochastic encoding for the same $\hat{\mbf{z}}_0(\mbf{y})$
% %\end{theorem}
% \begin{lemma}
% \label{thm:smallvariance}
% Let $\tilde{\mbf{z}}_t$ and $\hat{\mbf{z}}_t$ denote the stochastically encoded and resampled image of $\hat{\mbf{z}}_0(\mbf{y})$, respectively. If $\text{VAR}(\mbf{z}'_t) > 0$, then we have that $\text{VAR}(\hat{\mbf{z}}_t) < \text{VAR}(\tilde{\mbf{z}}_t)$.
% \end{lemma}
% By Theorem~\ref{thm:unbias}, we have that stochastic resampling is consistent with the prior of the pre-trained diffusion model, yielding no bias in the mapping step.
% %As a result, we incorporate both the data(measurement) consistency and prior consistency in our proposed ReSample algorithm.
% Theorem~\ref{thm:smallvariance} proves that we can both effectively reduce and control the variance of our measurement-consistent sample. Following our theory, we empirically observe that the samples from stochastic resampling reconstructs signals that are less noisier than stochastic encoding, for which we show in Section~\ref{sec:resample_exp}.
